Disaggregated Memory with SmartNIC Offloading: a Case Study on Graph Processing

Disaggregated memory breaks the boundary of monolithic servers to enable memory provisioning on demand. Using network-attached memory to provide memory expansion for memory-intensive applications on compute nodes can improve the overall memory utilization on a cluster and reduce the total cost of ownership. However, current software solutions for leveraging network-attached memory must consume resources on the compute node for memory management tasks. Emerging off-path smartNICs provide general-purpose programmability at low-cost low-power cores. This work provides a general architecture design that enables network-attached memory and offloading tasks onto off-path programmable SmartNIC. We provide a prototype implementation called SODA on Nvidia BlueField DPU. SODA adapts communication paths and data transfer alternatives, pipelines data movement stages, and enables customizable data caching and prefetching optimizations. We evaluate SODA in five representative graph applications on real-world graphs. Our results show that SODA can achieve up to 7.9x speedup compared to node-local SSD and reduce network traffic by 42% compared to disaggregated memory without SmartNIC offloading at similar or better performance.

==> overview.tex <==
\section{Overview}
\tool consists of three agents, running on the host, DPU, and memory node, respectively. Figure~\ref{fig:design} depicts their main components and interactions. The \textbf{host agent} manages a memory buffer for staging data from the memory node. Its main tasks include issuing requests for data and evicting data when the buffer is full. The \textbf{DPU agent} is tasked with receiving and processing requests from the host, aggregating and forwarding requests to the memory node, managing and optimizing data movement between the compute and memory nodes. It also leverages its local DRAM to prefetch and cache data. A DPU agent may handle multiple host agents on a compute node. The \textbf{memory agent} is deployed on the memory node and it only handles simple tasks like reserving and freeing memory resources.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/design.pdf}
    \caption{\tool consists of agents on the host, SmartNIC SoC (DPU), and memory server. Memory objects in the application process's virtual space can be backed by network-attached memory. \tool agents transparently handle tasks for memory management and data movement for the application.}
    \label{fig:design}
\end{figure}

